Single Ground Truth Is Not Enough: Adding Flexibility to Aspect-Based Sentiment Analysis Evaluation

Aspect-based sentiment analysis (ABSA) is a challenging task of extracting sentiments along with their corresponding aspects and opinion terms from the text. The inherent subjectivity of span annotation makes variability in the surface forms of extracted terms, complicating the evaluation process. Traditional evaluation methods often constrain ground truths (GT) to a single term, potentially misrepresenting the accuracy of semantically valid predictions that differ in surface form. To address this limitation, we propose a novel and fully automated pipeline that expands existing evaluation sets by adding alternative valid terms for aspect and opinion. Our approach facilitates an equitable assessment of language models by accommodating multiple-answer candidates, resulting in enhanced human agreement compared to single-answer test sets (achieving up to a 10\%p improvement in Kendall's Tau score). Experimental results demonstrate that our expanded evaluation set helps uncover the capabilities of large language models (LLMs) in ABSA tasks, which is concealed by the single-answer GT sets. Consequently, our work contributes to the development of a flexible evaluation framework for ABSA by embracing diverse surface forms to span extraction tasks in a cost-effective and reproducible manner. Our code and dataset is open at https://github.com/dudrrm/zoom-in-n-out-absa.

==> tables/llm_comparison.tex <==
% \hspace{3mm}

% \begin{table*}[]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|ccc|ccc|ccc|ccc}
% \toprule
%  & \multicolumn{3}{c|}{\textbf{ASQP-R15}} & \multicolumn{3}{c|}{\textbf{ASQP-R16}} & \multicolumn{3}{c|}{\textbf{ACOS-Laptop}} & \multicolumn{3}{c}{\textbf{ACOS-Rest}} \\
%  & \textbf{Llama\textsuperscript{$\dagger$}} & \textbf{GPT} & \textbf{Gemini} & \textbf{Llama\textsuperscript{$\dagger$}} & \textbf{GPT} & \textbf{Gemini} & \textbf{Llama\textsuperscript{$\dagger$}} & \textbf{GPT} & \textbf{Gemini} & \textbf{Llama\textsuperscript{$\dagger$}} & \textbf{GPT} & \textbf{Gemini} \\

% \midrule
% \textbf{\#Pred} & 1501.96\small{$\pm$600} & 990 & 956 & 1033 & 997 & 929 & 1236 & 1680 & 1262 & 1510 & 955 & 973 \\
% \textbf{\#TP} & 322 & 418 & 439 & 377 & 460 & 511 & 235 & 690 & 488 & 428 & 484 & 502 \\
% % \hline
% \rowcolor[HTML]{FFCE93}
% % \rowcolor[HTML]{FFFC9E} 
% \textbf{\hspace{3mm}\#Implicit} & 71 & {\ul 107} & \textbf{117} & \textbf{93} & 75 & {\ul 85} & 5 & {\ul 56} & \textbf{122} & {\ul 118} & 96 & \textbf{125} \\
% \rowcolor[HTML]{DAE8FC}
% \textbf{\hspace{3mm}\#Explicit} & 251 & {\ul 311} & \textbf{322} & 284 & {\ul 385} & \textbf{426} & 230 & \textbf{634} & {\ul 366} & 310 & \textbf{388} & {\ul 377} \\

% \\[-2ex]
% \hline
% \textbf{F1 score} & 36.2 & {\ul 46.83} & \textbf{50.14} & 41.16 & {\ul 51.22} & \textbf{59.14} & 19.61 & \textbf{48.57} & {\ul 40.28} & 35.28 & {\ul 51.74} & \textbf{53.15} \\

% \\[-2ex]
% \hline
% \rowcolor[HTML]{EFEFEF} 
% \textit{Avg. F1} & \textit{30.08} & \textit{43.12} & \textit{47.23} & \textit{33.22} & \textit{47.52} & \textit{56.84} & \textit{14.73} & \textit{30.81} & \textit{36.55} & \textit{27.41} & \textit{45.1} & \textit{47.35}
%  \\
% \bottomrule
% \end{tabular}%
% }
% \caption{Evaluation on our test set where each model is the best model in naive prediction setting.}
% \label{tab:appendix-gpt-vs-gemini}
% \end{table*}


\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|ccc|ccc|ccc|ccc}
\toprule
 & \multicolumn{3}{c|}{\textbf{ASQP-R15}} & \multicolumn{3}{c|}{\textbf{ASQP-R16}} & \multicolumn{3}{c|}{\textbf{ACOS-Laptop}} & \multicolumn{3}{c}{\textbf{ACOS-Rest}} \\
 & \textbf{Llama\textsuperscript{$\ddagger$}} & \textbf{GPT} & \textbf{Gemini} & \textbf{Llama\textsuperscript{$\ddagger$}} & \textbf{GPT} & \textbf{Gemini} & \textbf{Llama\textsuperscript{$\ddagger$}} & \textbf{GPT} & \textbf{Gemini} & \textbf{Llama\textsuperscript{$\ddagger$}} & \textbf{GPT} & \textbf{Gemini} \\
\midrule  
\textbf{\# Pred} & 1502\small{$\pm$600} & 993\small{$\pm$27} & 999\small{$\pm$56} & 1471\small{$\pm$487} & 1040\small{$\pm$65} & 944\small{$\pm$24} & 1497\small{$\pm$407} & 1496\small{$\pm$186} & 1292\small{$\pm$56} & 1913\small{$\pm$600} & 1040\small{$\pm$80} & 957\small{$\pm$15} \\
\textbf{\# TP} & 333\small{$\pm$34} & 386\small{$\pm$14} & 423\small{$\pm$12} & 365\small{$\pm$27} & 436\small{$\pm$15} & 495\small{$\pm$13} & 192\small{$\pm$22} & 409\small{$\pm$62} & 448\small{$\pm$23} & 376\small{$\pm$37} & 440\small{$\pm$25} & 443\small{$\pm$40} \\
\rowcolor[HTML]{EFEFEF} 
\textbf{\hspace{2mm}\# Imp.} & 89\small{$\pm$16} & 89\small{$\pm$8} & \textbf{108\small{$\pm$5}} & \textbf{92\small{$\pm$17}} & 74\small{$\pm$4} & 88\small{$\pm$4} & 7\small{$\pm$5} & 43\small{$\pm$15} & \textbf{107\small{$\pm$16}} & 98\small{$\pm$28} & 86\small{$\pm$12} & \textbf{116\small{$\pm$16}} \\
\rowcolor[HTML]{EFEFEF} 
\textbf{\hspace{2mm}\# Exp.} & 244\small{$\pm$27} & 296\small{$\pm$12} & \textbf{315\small{$\pm$10}} & 273\small{$\pm$28} & 362\small{$\pm$16} & \textbf{408\small{$\pm$11}} & 186\small{$\pm$22} & \textbf{365\small{$\pm$59}} & 341\small{$\pm$14} & 278\small{$\pm$28} & \textbf{354\small{$\pm$19}} & 328\small{$\pm$26} \\
\midrule
\textbf{F1 score} & 30.1\small{$\pm$5} & 43.1\small{$\pm$2} & \textbf{47.2\small{$\pm$2}} & 33.2\small{$\pm$5} & 47.5\small{$\pm$3} & \textbf{56.8\small{$\pm$2}} & 14.7\small{$\pm$2} & 30.8\small{$\pm$4} & \textbf{36.5\small{$\pm$2}} & 27.4\small{$\pm$5} & 45.1\small{$\pm$4} & \textbf{47.4\small{$\pm$4}} \\
\bottomrule
\end{tabular}%
}
\caption{Details of LLMs' performance on our test set. The first two rows represent the average and standard deviation of the number of predictions (\# Pred) and true-positive predictions (\# TP). In the true-positive predictions, we count the implicit (\# Imp.) and explicit (\# Exp.) cases, where the implicit case indicates when the predicted quadruple includes ``null'' in the aspect or opinion term. The models are Llama-2-70B with constrained decoding, GPT-3.5-Turbo, and Gemini-v1.5-Pro, respectively.}

\label{tab:appendix-llm-comparison}
\end{table*}


